$O(1)$-Round MPC Algorithms for Multi-dimensional Grid Graph Connectivity, EMST and DBSCAN

In this paper, we investigate three fundamental problems in the Massively Parallel Computation (MPC) model: (i) grid graph connectivity, (ii) approximate Euclidean Minimum Spanning Tree (EMST), and (iii) approximate DBSCAN. Our first result is a $O(1)$-round Las Vegas (i.e., succeeding with high probability) MPC algorithm for computing the connected components on a $d$-dimensional $c$-penetration grid graph ($(d,c)$-grid graph), where both $d$ and $c$ are positive integer constants. In such a grid graph, each vertex is a point with integer coordinates in $\mathbb{N}^d$, and an edge can only exist between two distinct vertices with $\ell_\infty$-norm at most $c$. To our knowledge, the current best existing result for computing the connected components (CC's) on $(d,c)$-grid graphs in the MPC model is to run the state-of-the-art MPC CC algorithms that are designed for general graphs: they achieve $O(\log \log n + \log D)$[FOCS19] and $O(\log \log n + \log \frac{1}{\lambda})$[PODC19] rounds, respectively, where $D$ is the {\em diameter} and $\lambda$ is the {\em spectral gap} of the graph. With our grid graph connectivity technique, our second main result is a $O(1)$-round Las Vegas MPC algorithm for computing approximate Euclidean MST. The existing state-of-the-art result on this problem is the $O(1)$-round MPC algorithm proposed by Andoni et al.[STOC14], which only guarantees an approximation on the overall weight in expectation. In contrast, our algorithm not only guarantees a deterministic overall weight approximation, but also achieves a deterministic edge-wise weight approximation.The latter property is crucial to many applications, such as finding the Bichromatic Closest Pair and DBSCAN clustering. Last but not the least, our third main result is a $O(1)$-round Las Vegas MPC algorithm for computing an approximate DBSCAN clustering in $O(1)$-dimensional space.

==> algorithm1.tex <==
\begin{algorithm}[t]
\caption{Storage location of non-empty neighbor grid}\label{algo:neiloc}
\KwData{A set of $m$ machines $(M_1,\ldots,M_m)$, each machine~$M_i$ contains points from $k^{(i)}$ grids $(g_1^{(i)},\cdots,g_{k^{(i)}}^{(i)})$, the storage location of the grid $g.\loc$ 
\KwResult{Given a non-empty grid~$g$, calculate the storage location of every $g'\in \Nei_g$}
\For{machine $M_i$, $i\in[1,m]$ simultaneously}{
\For{each support grid~$g_j$, $j\in [1,k^{(i)}]$}{
    Build $4$-tuples $(g_j.\coord,M_i, g'.\coord,g'.\loc)$ for each $g'\in \Nei_{gj}$\;
    //the fourth term is a placeholder with value NULL now
}
}
Invoke a sorting algorithm for all of the $4$-tuples based on the $g'.\coord$\;
\For{machine $M_i$, $i\in[1,m]$ simultaneously}{
    Broadcast the minimal and maximal $g'.\coord$ \;
    //each machine also receives that information during the communication phase\;
    \For{each grid $g_j$, $j\in [1,k^{(i)}]$}{
    Send the $2$-tuple $(g_j.\coord,g_j.\loc)$ to the machines $M$ s.t. $g_j.\coord \in [M.\min(g'.\coord),M.\max(g'.\coord)]$\;
}
//each machine also receives the 2-tuple during the communication phase\;
Merge the 2-tuple with 4-tuple to fill in the placeholder\;
\For{each 4-tuple with $g'.\loc!=\text{NULL}$}{
    Send the 4-tuple back to $M_i$\;
}
//each machine receive the backward 4-tuple during the communication phase\;
}


\end{algorithm}


==> emstalgo.tex <==
\begin{small}
\begin{algorithm}
	\caption{MPC EMST Algorithm}\label{algo:emst}
	\KwData{$V$ is the input vertex set, $s=|V|^\alpha$ is the MPC local memory, $\rho$ is the EMST approximate parameter
	}
	initialize $V_1\leftarrow V$, $l_1\leftarrow s^{1/d^3}$ \;
        let $i$ denote the loop number for the following while loop, $\T\leftarrow \emptyset$ denote the result set\;
	\While{$l_i<\Delta$}{
        solve MST problem on $G_i=(V_i,\E_i(\cdot,\cdot))$, the result is denoted by $\T_i$\;
        revert edges in $\T_i$ to their original form $\T'_i$, $\T\leftarrow\T\cup \T'_i$\;
        compress the vertices into $V_{i+1}$\;
	}
	output $\T$ as the result\;
\vspace{-1mm}
\end{algorithm}
\end{small}
